PreFair: Privately Generating Justifiably Fair Synthetic Data

When a database is protected by Differential Privacy (DP), its usability is limited in scope. In this scenario, generating a synthetic version of the data that mimics the properties of the private data allows users to perform any operation on the synthetic data, while maintaining the privacy of the original data. Therefore, multiple works have been devoted to devising systems for DP synthetic data generation. However, such systems may preserve or even magnify properties of the data that make it unfair, endering the synthetic data unfit for use. In this work, we present PreFair, a system that allows for DP fair synthetic data generation. PreFair extends the state-of-the-art DP data generation mechanisms by incorporating a causal fairness criterion that ensures fair synthetic data. We adapt the notion of justifiable fairness to fit the synthetic data generation scenario. We further study the problem of generating DP fair synthetic data, showing its intractability and designing algorithms that are optimal under certain assumptions. We also provide an extensive experimental evaluation, showing that PreFair generates synthetic data that is significantly fairer than the data generated by leading DP data generation mechanisms, while remaining faithful to the private data.

==> mnist_extend.tex <==
Similar to PrivBayes \cite{PrivBays} MST \cite{RyanMnist} is another mechanism for creating private synthetic data. Similar to PrivBayes MST generates data in two steps. First it privately constructs a minimum spanning tree across all attributes. It does this by first measuring one way marginals then using Private-PGM\cite{McKennaSM19} to estimate each of the two way Marginals. From there it uses a private version of Kruskal's algorithm, where each edge is chosen using the exponential mechanism, in order to construct the MST. From there, like privbayes it uses samples directly from the MST by imposing conditional dependencies between neighboring nodes. For concreteness we show the orignal MST mechanism in Algorithm \ref{Algo:MST}. 
Unlike PrivBayes MST doesn't satisfy differential privacy directly instead choosing to satisfy Renyi Differential Privacy \cite{RenyiDP} and use that to derive a traditional differentially private guarantee. MST often performs better than most other DP-synthetic data mechanisms \cite{SynthBenchmark} and has several other advantages as well. In addition MST can be seeded with either public knowledge data (if it is available) or sets of edges that must be present in the final resulting graphical model. Likewise it has been shown to widely be the best performing differentially private synthetic data mechanism \cite{SynthBenchmark}. %
We begin by showing that the general greedy mechanism for generating a minimum spanning tree does not work in this context then show that finding the optimal minimum spanning tree that satisfies \cref{thrm:bayes_path}. From there similar to the case of PrivBayes we discuss both an optimal dynamic programming solution as well as a more efficient greedy solution which satisfies \cref{thrm:just_fair_condition}. For concreteness we repeat the original MST algorithm in Algorithm \ref{Algo:MST}


==> notation.tex <==
\begin{tcolorbox}

\begin{align*}
D & & \text{Database} \\
\gA & & \text{Attributes of D} \\
P & & \text{Protected attributes of D} \\
A & & \text{Admissible attributes of D}\\
I & & \text{inadmissible attributes of D}\\
O & & \text{Outcome Attribute} \\
\epsilon & & \text{Privacy budget} \\
\gN & & \text{Bayes Net}\\
\lambda & & \text{Degree of Bayes net} \\
X_i & & \text{ith node in a bayes net}\\
\delta_i & & \text{Descendants of node i}\\
\Pi_i & & \text{Parents of node i}\\
n & & \text{Number of individuals in} D
\end{align*} 



\end{tcolorbox}


==> overview.tex <==
\section{Solution Overview}

First we demonstrate in \cref{sec:3SAT} that finding the optimal MST structure in the general case is NP hard via a reduction from 3-SAT. Similar results have been shown before in other settings \cite{InterFair} however we extend those results the restricted case of MST graphical models. From there in \cref{sec:optimal} we show an exponential time solution to find the optimal MST. We then demonstrate in \cref{sec:greedy} a greedy algorithm which generates a fair MST in linear time. This mechanism produces data which performs well in practice while also incurring a smaller privacy loss for the same amount of noise. We also demonstrate a particular special case where the greedy mechanism does result in the optimal MST. In \cref{sec:experiments} we then evaluate our mechanisms to the current state of the art differentially private synthetic data generation. In addition we evaluate the downstream fairness affects of synthetic data generated by our mechanisms.
% 
